SciClops: Detecting and Contextualizing Scientific Claims for Assisting Manual Fact-Checking

This paper describes SciClops, a method to help combat online scientific misinformation. Although automated fact-checking methods have gained significant attention recently, they require pre-existing ground-truth evidence, which, in the scientific context, is sparse and scattered across a constantly-evolving scientific literature. Existing methods do not exploit this literature, which can effectively contextualize and combat science-related fallacies. Furthermore, these methods rarely require human intervention, which is essential for the convoluted and critical domain of scientific misinformation. SciClops involves three main steps to process scientific claims found in online news articles and social media postings: extraction, clustering, and contextualization. First, the extraction of scientific claims takes place using a domain-specific, fine-tuned transformer model. Second, similar claims extracted from heterogeneous sources are clustered together with related scientific literature using a method that exploits their content and the connections among them. Third, check-worthy claims, broadcasted by popular yet unreliable sources, are highlighted together with an enhanced fact-checking context that includes related verified claims, news articles, and scientific papers. Extensive experiments show that SciClops tackles sufficiently these three steps, and effectively assists non-expert fact-checkers in the verification of complex scientific claims, outperforming commercial fact-checking systems.

==> 03-corpus.tex <==
% !TEX root = main.tex

\section{Data Collection}
\label{sec:corpus}

%\note[from=ChaTo]{Next paragraph says there is no collection but what about the SciLens one? Perhaps we could say we follow a similar methodology, or we merge SciLens's dataset with a new collection.}
%Since there is no data collection available, that combines scientific papers, news articles and social media postings, we introduce a custom one.
%

As explained above, our method is based on heterogeneous information coming from \emph{social media postings}, \emph{news articles}, and \emph{scientific papers}.
%
In this section we explain the procedure we follow to obtain suitable data that includes scientific claims. %such data collection.
%similar to the approach proposed by \citet{DBLP:conf/www/Smeros0A19}.


\spara{Bottom-Up Procedure.}
Social media postings containing scientific claims are usually motivated by scientific news articles or scientific papers;
%
thus, we use these postings as our starting point. %which is why we call this a ``bottom-up'' procedure.
%We use social media as our starting point.
%
We harvest social media postings from \rurl{Spinn3r.com} using a set of seed keywords that we describe below.
%
Additionally to the text of each posting, we collect the number of interactions the posting has received i.e., other users \emph{re-postings} and \emph{likes}.
%
Finally, we discard postings without outgoing URLs or with spam/unreachable URLs.



In the second step, we use a standard crawling method in which we visit, download, and parse the pages pointed by the URLs found in the social media postings.
%
%We consider that these pages contain news-worthy information since their
The majority of these pages comes from mainstream news outlets (e.g., \rurl{theguardian.com} or \rurl{popsci.com}), as well as from alternative blogging platforms (e.g., \rurl{mercola.com} or \rurl{foodbabe.com}).
%\todo[from=ChaTo]{The list above could be defined more precisely, e.g., indicating from where those outlets were collected, how many are there, and perhaps some examples.}
In the following sections, we will refer to this middle-layer of our data collection simply as \emph{news articles}.


In the last step of our procedure, we search within the news articles for references to scientific papers.
%
The scientific papers are peer-reviewed or gray literature\footnote{\url{https://en.wikipedia.org/wiki/Grey_literature}} papers hosted at universities, academic publishers, or scientific repositories. %, or public institution (e.g., a public health institute).
%
We use a large list of academic sources consisting of:
\begin{inparaenum}[i)]
	\item the top-1000 universities in the world (retrieved from \rurl{CWUR.org}), and
	\item about $150$ academic databases (retrieved from Wikipedia\footnote{\url{https://en.wikipedia.org/wiki/List\_of\_academic\_databases\_and\_search\_engines}}), including Scopus, PubMed, and JSTOR, among many others.
\end{inparaenum}
%
For these scientific papers, we extract their title and full content.
%
Finally, we discard from our data collection unparsable and pay-walled scientific papers, as well as news articles that do not contain any reference to scientific papers.


\spara{Seed Keywords.}
%
The procedure we described is domain-agnostic.
%
The theme and the language of our data collection depend only on the selection of the seed keywords.
%
In the context of this paper, we choose English keywords related to health and nutrition, including scientific and common names of food families, nutrients, conditions, and diseases.
%
Specifically, we acquired this set of seed keywords from \rurl{NutritionFacts.org}, a non-commercial website that provides scientific information on healthy eating.
%
The $\textasciitilde1.5K$ acquired keywords cover a broad spectrum of subtopics and contain terms from ``abdominal pain'' and ``appendicitis'' to ``zinc'' and ``zoonotic disease''.
%


\spara{Final Data Collection.}
%
Our data collection has the form of a directed graph, from social media postings to news articles to scientific papers, where edges denote a hyperlink connection.
%
For the narrow domain of \emph{health and nutrition} and before the outbreak of \emph{COVID-19} (in late 2019),
%\note[from=ChaTo]{I'm noting the collection is from late 2019 to emphasize it is pre-COVID but not ancient.}
%
we acquired $\textasciitilde49K$ social media postings, referencing $\textasciitilde12K$ news articles from $\textasciitilde3.5K$ news outlets, referencing $\textasciitilde24K$ scientific papers.
%
The data collection will be available for research purposes with the camera-ready version of this paper.


In the following sections we use:
\begin{inparaenum}[i)]
	\item the \emph{social media postings} and the \emph{news articles} for extracting potential scientific claims (\S\ref{sec:extraction}),
	\item the extracted claims and the \emph{scientific papers} for computing the multi-modal clusters (\S\ref{sec:clustering}), and
	\item meta-information such as the popularity of \emph{social media postings} and the reputation of \emph{news outlets}, for ranking emerging scientific claims (\S\ref{sec:verification}).
\end{inparaenum}

